DisCo-Diff: Enhancing Continuous Diffusion Models with Discrete Latents

Diffusion models (DMs) have revolutionized generative learning. They utilize a diffusion process to encode data into a simple Gaussian distribution. However, encoding a complex, potentially multimodal data distribution into a single continuous Gaussian distribution arguably represents an unnecessarily challenging learning problem. We propose Discrete-Continuous Latent Variable Diffusion Models (DisCo-Diff) to simplify this task by introducing complementary discrete latent variables. We augment DMs with learnable discrete latents, inferred with an encoder, and train DM and encoder end-to-end. DisCo-Diff does not rely on pre-trained networks, making the framework universally applicable. The discrete latents significantly simplify learning the DM's complex noise-to-data mapping by reducing the curvature of the DM's generative ODE. An additional autoregressive transformer models the distribution of the discrete latents, a simple step because DisCo-Diff requires only few discrete variables with small codebooks. We validate DisCo-Diff on toy data, several image synthesis tasks as well as molecular docking, and find that introducing discrete latents consistently improves model performance. For example, DisCo-Diff achieves state-of-the-art FID scores on class-conditioned ImageNet-64/128 datasets with ODE sampler.

==> sections/4_related_work.tex <==
\section{Related Work}
Our work builds on DMs~\cite{ho2020ddpm,song2020score,sohl2015deep}, which have been widely used not only for image generation~\cite{dhariwal2021diffusion,saharia2022photorealistic,ramesh2022dalle2,rombach2021highresolution}, but also for video~\cite{blattmann2023videoldm,singer2023makeavideo,ho2022imagen}, 3D~\cite{nichol2022pointe,kim2023nfldm,poole2023dreamfusion,schwarz2023wildfusion} and 4D~\cite{singer2023mav3d,ling2024align,bahmani20234dfy} synthesis, as well as in various other domains, including, for instance, molecular docking and protein design~\cite{corso2023diffdock,yim2023framediff,ingraham2022chroma,watson2023rfdiffusion}. In the DM literature, latent variables have been most popular as part of latent diffusion models, where a DM is trained in a compressed, usually continuous, latent space~\cite{rombach2021highresolution,vahdat2021score}. In contrast, DisCo-Diff leverages \textit{discrete} latent variables and uses them to augment a DM. The first models using discrete latent variables for high-dimensional generative modeling tasks include Boltzmann machines~\cite{salakhutdinov2009deep,hinton2012practical} and early discrete variational autoencoders~\cite{rolfe2017discrete,vahdat2018dvae,vahdat2018dvaepp}. More recently, a variety of works encode images into large 2D spatial grids of discrete tokens with vector quantization or similar techniques~\cite{vandenoord2017vqvae,esser2021vqgan,ramesh2021dalle,chang2022maskgit,yu2022scaling,pernias2023wuerstchen,chang2023muse}. As discussed, these models typically require a very large number of tokens and rely on large codebooks, which makes modeling their distribution challenging. DisCo-Diff, in contrast, leverages only few discrete latents with small codebooks that act in harmony with the additional continuous DM. 

There are previous related works that also condition DMs on auxiliary encodings. \citet{preechakul2021diffusion} augment DMs with non-spatial latent variables, but their latents are continuous and high-dimensional, which makes training their latent DM more challenging. This is precisely what we avoid by instead using low-dimensional and discrete latents. Moreover, they focus on semantic face image manipulation, not high-quality synthesis for challenging, diverse datasets. 
% We show how discrete latents boost generative performance itself. 
% \citet{harvey2023visual} and \citet{li2023selfconditioned} use the representation inferred by existing large-scale semantic image encoders, such as CLIP~\cite{...} or based on MoCo~\cite{...}, for conditioning in a DM. Hence, these approaches are restricted to image generation, where such pre-trained encoders are available. 

\citet{harvey2023visual} use the representations of a pre-trained CLIP image encoder~\cite{radford2021clip} for conditioning a DM and learn another DM over the CLIP embeddings for sampling. Similarly, \citet{bao2022conditional} and \citet{hu2023SelfGuidedDM} use clustered MoCo-based~\cite{he2020moco} and clustered DINO-based~\cite{caron2021dino} features, respectively, for conditioning. Hence, these three approaches are strictly limited to image synthesis, where such encoders, pre-trained on large-scale datasets, are available. In contrast, we purposefully avoid the use of pre-trained networks and learn the discrete latents jointly with the DM, making our framework universally applicable.
Another related work is InfoDiffusion~\cite{wang2023infodiffusion}, which also conditions DMs on discrete latent variables. However, contrary to DisCo-Diff, this work focuses on learning disentangled representations, similar to $\beta$-VAEs~\cite{higgins2017betavae}, primarily for low-resolution face synthesis. It uses a mutual information-based objective and does not focus on diverse and high-quality synthesis of complex data such as ImageNet. 

In contrast to the above works, we show how discrete latent variables boost generative performance itself and we significantly outperform these works in complex and diverse high-quality synthesis. Furthermore, we motivate DisCo-Diff fundamentally, with reduced ODE curvature and model complexity, providing a new and complementary perspective.\looseness=-1

\kk{If we include protein or docking experiments, we need a short paragraph on corresponding related work, too.}
% Karsten: I did not mention li2023selfconditioned, because I think we can consider this work concurrent.

% Quantitatively, we outperform this work quantitatively by a large margin.
% Moreover, in contrast to the above works, we motivate our design choices from a fundamental model complexity and generative ODE curvature perspective.
% Our framework can be interpreted as a modern discrete variational autoencoder with a DM decoder.
% Discrete latent variable models with spatial grids (VQGAN et al.)
% Old discrete variational autoencoder literature
% Continuous latent variable diffusion models, i.e., LDM/LSGM et al.
% Most related to us: InfoDiffusion~\cite{wang2023infodiffusion} 
% Related to that: InfoVAE/InfoGAN type works?
% ``Cont. latent version'': \cite{preechakul2021diffusion}
% Use of pre-trained image encoder networks \cite{harvey2023visual,li2023selfconditioned}
% The paper that uses clustering to get extra conditioning (was it ``Why Are Conditional Generative Models Better Than Unconditional Ones?''?) 
% Some works utilize the clustered label of features from pre-trained encoders. For example,   \cite{bao2022conditional} uses the clustered label of the Moco feature, and \cite{hu2023SelfGuidedDM}  uses the clustered label of the DINO feature as conditional input. Instance-conditioned GAN.
% Some general diffusion model paragraph.
% (maybe put extended version in Appendix, and only discuss most relevant works in main paper)
